Physics-Informed Surrogates for Temperature Prediction of Multi-Tracks in Laser Powder Bed Fusion

Modeling plays a critical role in additive manufacturing (AM), enabling a deeper understanding of underlying processes. Parametric solutions for such models are of great importance, enabling the optimization of production processes and considerable cost reductions. However, the complexity of the problem and diversity of spatio-temporal scales involved in the process pose significant challenges for traditional numerical methods. Surrogate models offer a powerful alternative by accelerating simulations and facilitating real-time monitoring and control. The present study presents an operator learning approach that relies on the deep operator network (DeepONet) and physics-informed neural networks (PINN) to predict the three-dimensional temperature distribution during melting and consolidation in laser powder bed fusion (LPBF). Parametric solutions for both single-track and multi-track scenarios with respect to tool path are obtained. To address the challenges in obtaining parametric solutions for multi-track scenarios using DeepONet architecture, a sequential PINN approach is proposed to efficiently manage the increased training complexity inherent in those scenarios. The accuracy and consistency of the model are verified against finite-difference computations. The developed surrogate allows us to efficiently analyze the effect of scanning paths and laser parameters on the thermal history.

==> domain.tex <==
%% Creator: Inkscape 1.3.2 (091e20e, 2023-11-25, custom), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'Domain1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{263.04000092bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.76368612)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{Domain1.pdf}}%
    \put(0.07706684,0.38408088){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1 mm\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{Domain1.pdf}}%
    \put(0.54987323,0.07198208){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}2 mm\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{Domain1.pdf}}%
    \put(0.76975439,0.42367548){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1.5 mm\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{Domain1.pdf}}%
    \put(0.54987323,0.35147353){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1 mm\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{Domain1.pdf}}%
    \put(0.68408736,0.38175178){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Track 1\end{tabular}}}}%
    \put(0.63750544,0.4283337){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Track 2\end{tabular}}}}%
    \put(0.59092353,0.47491559){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Track 3\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{Domain1.pdf}}%
    \put(0.47821715,0.67288872){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Laser\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{Domain1.pdf}}%
    \put(0.26572357,0.08595665){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}x\end{tabular}}}}%
    \put(0.18653433,0.11856397){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}y\end{tabular}}}}%
    \put(0.23544533,0.1604877){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}z\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=8]{Domain1.pdf}}%
  \end{picture}%
\endgroup%


==> results/multi-track-soft.tex <==
\begin{figure}[p]
    \centering
    \begin{subfigure}{0.65\textwidth}
    \includegraphics[width=\textwidth]{Figures/all_path_pinn_fd.png}
    \caption{}
    \label{fig:all_path_a}
    \end{subfigure}
    \begin{subfigure}{0.85\textwidth}
    \includegraphics[width=\textwidth]{Figures/all_path_meltpool.pdf}
    \caption{}
    \label{fig:all_path_b}
    \end{subfigure}
    
    \caption{Comparison of the calculated temperature and meltpool dimensions for all paths in multi-track scenarios. (a): PINN solution vs. reference (FD) solution. 5 \% relative error zone is indicated by light red color. (b): Comparison of Meltpool sizes for each path.}
    \label{fig:all_compare}
\end{figure}

\begin{figure}[p]
    \centering
    \begin{subfigure}{0.85\textwidth}
    \includegraphics[width=\textwidth]{Figures/all_path_xy.pdf}
    \caption{$xy$-plane}
    \label{fig:multi_a}
    \end{subfigure}
    \begin{subfigure}{0.85\textwidth}
    \includegraphics[width=\textwidth]{Figures/all_path_xz.pdf}
    \caption{$xz$-plane}
    \label{fig:multi_b}
    \end{subfigure}
    
    \caption{Comparison between the PINN predictions and finite-difference solutions for all paths in both $xy-$ and $xz-$ planes.}
    \label{fig:all_compare_T}
\end{figure}


\begin{figure}[p]
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/cooling.pdf}
    \caption{Comparison of the temperature history for a point within the meltpool during the cooling phase. Error bars represent 5\% error with respect to FD solution.}
    \label{fig:cooling}
\end{figure}

\begin{figure}[p]
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/all_re.png}
    \caption{Comparison of the final cooling temperature across the meltpool region.}
    \label{fig:cooling_all}
\end{figure}
